Understanding AI Trustworthiness: A Scoping Review of AIES & FAccT Articles

Background: Trustworthy AI serves as a foundational pillar for two major AI ethics conferences: AIES and FAccT. However, current research often adopts techno-centric approaches, focusing primarily on technical attributes such as reliability, robustness, and fairness, while overlooking the sociotechnical dimensions critical to understanding AI trustworthiness in real-world contexts. Objectives: This scoping review aims to examine how the AIES and FAccT communities conceptualize, measure, and validate AI trustworthiness, identifying major gaps and opportunities for advancing a holistic understanding of trustworthy AI systems. Methods: We conduct a scoping review of AIES and FAccT conference proceedings to date, systematically analyzing how trustworthiness is defined, operationalized, and applied across different research domains. Our analysis focuses on conceptualization approaches, measurement methods, verification and validation techniques, application areas, and underlying values. Results: While significant progress has been made in defining technical attributes such as transparency, accountability, and robustness, our findings reveal critical gaps. Current research often predominantly emphasizes technical precision at the expense of social and ethical considerations. The sociotechnical nature of AI systems remains less explored and trustworthiness emerges as a contested concept shaped by those with the power to define it. Conclusions: An interdisciplinary approach combining technical rigor with social, cultural, and institutional considerations is essential for advancing trustworthy AI. We propose actionable measures for the AI ethics community to adopt holistic frameworks that genuinely address the complex interplay between AI systems and society, ultimately promoting responsible technological development that benefits all stakeholders.

==> preamble/packages.tex <==
\RequirePackage[
  datamodel=acmdatamodel,
  style=acmauthoryear,
  backend=biber,
  giveninits=true
  ]{biblatex}

\renewcommand*{\bibopenbracket}{(}
\renewcommand*{\bibclosebracket}{)}

\usepackage{acronym}
\usepackage{xspace}
\usepackage[skip=1mm]{caption}
\usepackage{tikz}
\usetikzlibrary{mindmap}
\usepackage{todonotes}
\usepackage[inline]{enumitem}
% \usepackage{hyperref} # AAAI does not allow it

\usepackage{subcaption}
\usepackage{booktabs}

% These are recommended to typeset algorithms but not required. See the subsubsection on algorithms. Remove them if you don't have algorithms in your paper.
\usepackage{algorithm}
\usepackage{algorithmic}

\usepackage{rotating} 

%
% These are are recommended to typeset listings but not required. See the subsubsection on listing. Remove this block if you don't have listings in your paper.
\usepackage{newfloat}
\usepackage{listings}
\DeclareCaptionStyle{ruled}{labelfont=normalfont,labelsep=colon,strut=off} % DO NOT CHANGE THIS
\lstset{%
	basicstyle={\footnotesize\ttfamily},% footnotesize acceptable for monospace
	numbers=left,numberstyle=\footnotesize,xleftmargin=2em,% show line numbers, remove this entire line if you don't want the numbers.
	aboveskip=0pt,belowskip=0pt,%
	showstringspaces=false,tabsize=2,breaklines=true}
\floatstyle{ruled}
\newfloat{listing}{tb}{lst}{}
\floatname{listing}{Listing}
%
% Keep the \pdfinfo as shown here. There's no need
% for you to add the /Title and /Author tags.
\pdfinfo{
/TemplateVersion (2025.1)
}

\usepackage{bibentry}

\usepackage{ltablex}
\usepackage{ragged2e}
\renewcommand{\arraystretch}{1.15}
\keepXColumns


\usepackage{xcolor}   
\usepackage{soul}   
\usepackage{float}
\usepackage[skip=2pt]{caption}

==> sections/archived.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{|p{0.2\textwidth}|p{0.8\textwidth}|}
\hline
 \textbf{Keyword} & \textbf{Definition} \\
\hline
  & 1. Trustworthiness refers to the extent to which stakeholders can reasonably trust a model's outputs~\cite{Umang2020}. \\ % serial-number: 1
  & 2. A trustworthy AI system should be able to withstand scrutiny and thorough evaluation for potential risks and compliance with desired standards~\cite{Stephen2024}. \\ % ser: 2
  & 3. Trustworthiness is a property of the trustee (\eg AI model) that enables it to maintain a specific contract~\cite{Alon2021}. \\ % ser: 7
  & 4. Trustworthiness is related to the AI system's ability to accurately express its uncertainty~\cite{Sunnie2024a}. \\ % ser: 8
  \hline
\end{tabular}
\caption{For papers which explicitly define trustworthiness}
\label{tab:def}
\end{table}

\begin{table}[ht]
\centering
\begin{tabular}{|p{0.2\textwidth}|p{0.8\textwidth}|}
\hline
 \textbf{Keyword} & \textbf{Operationalization} \\
\hline
  &  \\
  \hline
\end{tabular}
\caption{For papers which explicitly operation trustworthiness}
\label{tab:op}
\end{table}

\begin{table}[ht]
\centering
\begin{tabular}{|p{0.2\textwidth}|p{0.8\textwidth}|}
\hline
 \textbf{Keyword} & \textbf{Conceptualization} \\
\hline
& 1. it is related to the transparency of the credit scoring mechanism and the ability of individuals to understand and act upon the information provided. (check? Definition?) \\ % ser: 3
& 2. Inferences made by AI systems based on facial images as acceptable, fair, justifiable, responsible, and appropriate \\ % ser: 4
& 3. Explainability is a property that makes AI trustworthy and is also part of what causes the belief that the AI is trustworthy, which, in turn, causes lower monitoring levels \\ % ser: 5 (not sure)
  & 4. How people perceive the anthropomorphization of technical systems descriptions is an important attribution of trustworthiness~\cite{Nanna2024}. \\ % ser: 6
  \hline
\end{tabular}
\caption{For papers which conceptualized trustworthiness}
\label{tab:concept}
\end{table}

\begin{table}[ht]
\caption{Top 5 Community Labels and Corresponding DOI Papers. Based on 236 N corpus. \sid{This table needs to be updated with proper references.} }
\label{tab:community_papers}
\centering
\begin{tabular}{lp{10cm}}
\toprule
\textbf{Community Label} & \textbf{DOI Papers} \\ \midrule
case, methods, participatory & 
10.1145/3630106.3658995 \\
& 10.1145/3600211.3604707 \\
& 10.1145/3593013.3594134 \\
& 10.1145/3600211.3604705 \\
& 10.1145/3442188.3445928 \\ 
\midrule

data, explainability, learning & 
10.1145/3593013.3594039 \\
& 10.1145/3351095.3375624 \\
& 10.1145/3461702.3462571 \\
& 10.1145/3600211.3604692 \\
& 10.1145/3593013.3594087 \\
& 10.1145/3593013.3594049 \\
& 10.1145/3461702.3462559 \\
& 10.1145/3351095.3372850 \\
& 10.1145/3351095.3372852 \\
& 10.1145/3600211.3604706 \\
& 10.1145/3630106.3658941 \\
& 10.1145/3514094.3534200 \\
& 10.1145/3630106.3659007 \\
& 10.1145/3442188.3445888 \\ 
\midrule

accountability, algorithmic, impact & 
10.1145/3593013.3594023 \\
& 10.1145/3593013.3594092 \\
& 10.1145/3531146.3533122 \\
& 10.1145/3593013.3593978 \\
& 10.1145/3630106.3658959 \\
& 10.1145/3531146.3533097 \\
& 10.1145/3461702.3462580 \\
& 10.1145/3630106.3658941 \\
& 10.1145/3461702.3462610 \\
& 10.1145/3593013.3594071 \\
& 10.1145/3531146.3533781 \\ 
\midrule

adoption, governance, health & 
10.1145/3600211.3604687 \\
& 10.1145/3531146.3533158 \\
& 10.1145/3630106.3658962 \\
& 10.1145/3351095.3372827 \\
& 10.1145/3514094.3534154 \\
& 10.1145/3593013.3594089 \\
& 10.1145/3461702.3462580 \\ 
\midrule

data, fairness, practitioners & 
10.1145/3531146.3533177 \\
& 10.1145/3630106.3658971 \\
& 10.1145/3531146.3533113 \\
& 10.1145/3593013.3594037 \\
& 10.1145/3630106.3658949 \\ 
\bottomrule
\end{tabular}
\end{table}

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/word_cloud_keywords.png}
    \caption{Enter Caption}
    \label{fig:enter-label}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{figures/values_co-occurance_network.png}
    \caption{A co-occurrence network graph showing the relationship between ISO trustworthiness dimensions within the final corpus ($N=43$).}
    \label{fig:values_network}
\end{figure}

\subsection{Impact of FAccT \& AIES Scholarship}
%Following the definition of impact by ref, we go through our corpus to see if and how they have impact. Table 4: Coding and categorization of FAccT affiliates’ notions of impact. - https://dl.acm.org/doi/pdf/10.1145/3531146.3533107

\todo[inline]{Is this also an output from the scoping review, or discussion? The place feels odd because the text does not directly engage with the results above. Is it results or discussion? If results, then what analysis did you use?}
FAccT and AIES has played a positive role in exposing its community to insights and ideas from other disciplines. In a recent work by \citet{laufer}, the authors report community views on deployment and broader impact. They categorized impact based on open-ended survey responses from FAccT affiliates in nine categories. These categories are (a) enhancing public literacy and awareness, (b) educating AI experts, (c) policy influence, (d) concrete benefits for impacted communities, (e) translation to practice, (f) buy-in from impacted communities, (g) intellectual paradigm shifts, (h) academic reach, and (i) political ramifications. Utilizing these categories, we will now analyze our corpus to study the broader impact of FAccT scholarship on AI trustworthiness.

One of the primary impacts of FAccT and AIES scholarship is the enhancement of public literacy regarding AI technologies. By critically examining the implications of AI systems, these conferences have fostered a greater understanding of the complexities involved in AI deployment, particularly concerning issues of fairness, accountability, and transparency. For instance, Knowles et al. argue that the rhetoric surrounding AI often marginalizes certain groups, creating a digital underclass that is perceived as 'undeserving' of trust in AI systems \cite{Bran2023}. Furthermore, Zhang and Dafoe highlight that public trust in institutions significantly influences the governance of AI, suggesting that informed citizens are better equipped to engage in discussions about AI regulation \cite{rayyan-64504662}.

Liao and Sundar emphasize the importance of communication in designing responsible AI systems that foster trust \cite{liao2022designing}. Such educational frameworks are critical for cultivating a workforce that prioritizes trustworthiness in AI design and implementation. Similarly,  \citet{lauren} discuss the necessity of transparency and accountability in AI systems, which have been instrumental in shaping policy discussions and \citet{benk2024twenty} empirical studies on certification labels for trustworthy AI provide actionable recommendations for policymakers seeking to establish standards for AI deployment.

The scholarship from FAccT and AIES has led to tangible benefits for communities adversely affected by AI systems. \citet{10.1145/3531146.3533218} highlight the detrimental effects of biased algorithms on marginalized groups, underscoring the need for equitable AI solutions. Similarly, \citet{Bran2023} argue that trust in AI systems is contingent upon addressing the structural inequalities that these technologies may exacerbate. By prioritizing community engagement, researchers and practitioners can foster a sense of ownership and trust among those impacted by AI, leading to more equitable outcomes.

The intellectual contributions of FAccT and AIES scholarship have catalyzed significant paradigm shifts in the understanding of AI trustworthiness. \citet{jacovi} formalize trust in AI systems, providing a foundational framework for rethinking how trust is conceptualized and measured in the context of AI. Similarly, academic reach of FAccT and AIES extends beyond the immediate community of AI researchers such as \citet{rayyan-64504624} studied accountability in AI use within public administrations, highlighting the need for cross-disciplinary engagement and \citet{rayyan-64504620} empirical assessment of AI governance challenges revealing the bureaucratic obstacles to effective AI regulation.

Overall, t











\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{figures/values_co-occurance_network.png}
    \caption{A co-occurrence network graph showing the relationship between ISO trustworthiness dimensions within the final corpus ($N=43$).}
    \label{fig:values_network}
\end{figure}


% \begin{figure}[ht!]
%     \centering
%     \includegraphics[width=0.75\linewidth]{figures/TEMP_louvain.png}
%     \caption{Enter Caption}
%     \label{fig:louvain}
% \end{figure}

% results with Louvain Community?

\header{Community Detection}
\sid{THIS PART IS STILL IN TODO. Xuelong: Please use S2ORC citation network where size of a given node is representative of the number of papers in the corresponding community. Edge thicknesses represents the volume of citations between the
respective communities}
We identify communities and their related topics using a version of the Louvain community detection method within the author network of our corpus. First, a network is constructed using co-authorship data, where nodes represents authors and edges denotes collaborations. Each connection is weighted by the frequency of joint publications. Second, using Louvain's algorithm, the network is partitioned into communities based on modularity optimization, grouping nodes to maximize intra-community connectivity while minimizing inter-community connections. Each community is labeled with the extracted top terms from the combined text data (title + abstract + keywords) of the associated articles, using a bag-of-words approach with the most frequent terms idenitified through a count vectorizer. Lastly, the network an their community IDs, top terms, and associated DOIs are visualized. The top five communities and their corresponding labels and papers are shown in Table \ref{tab:community_papers}. \textbf{Xuelong: I used DOIs just to illustrate, later I can write out author names. Especially when we definitively decided on the techniques}

Finally, we also performed some exploratory analysis on included papers. We constructed word clouds based on titles (Figure~\ref{fig:word_cloud_titles}) and abstracts of the articles (Figure~\ref{fig:word_cloud_abstract}). From the word cloud of titles, we could see the ``design'' and ``public'' are key highlights reflecting community focus on (re-)design of AI systems critically thinking about users, \textit{i.e.}, public and from the abstracts word cloud, it becomes apparent that our community's focus is on human in the loop and explanations as a prominent method for explaining inner workings of the AI system.

\subsection{Current Operational Challenges}
The implementation of AI trustworthiness faces several significant operational challenges. First, the industry trend toward limiting AI audits to black-box access substantially constrains evaluation scope and creates an imbalance favoring developers over other stakeholders \cite{Stephen2024}. This limitation is particularly problematic because localized explanations of model behavior, while helpful for understanding specific decisions, fail to provide comprehensive evidence of overall model trustworthiness.

Furthermore, \citet{ijerph19063641}  identified eight critical sources of risk affecting AI system trustworthiness: (a) fairness considerations in system outputs, (b) privacy preservation mechanisms, (c) degree of automation and human control, (d) task complexity and environmental context, (e) system transparency and explainability, (f) security measures and vulnerabilities, (g) hardware reliability and performance, and (h) overall technological maturity. Here, the first three deals with ethical aspects and remaining sources deals with various aspects that can influence the reliability and robustness of the AI system, and thus have a direct influence on the safety of the system. These risk factors interact within a complex socio-technical system where trustworthiness emerges from the interplay between developers, public authorities, and end-users. This interaction raises particular challenges for public authorities who must simultaneously regulate AI systems while increasingly relying on them for decision-making support.

Another critical perspective on stuyding AI trustworthiness is the need to address under-addressed issues such as the dominance of Western and Global Northern perspectives, the rapid diversification of AI application areas, and the reliance on exploratory research methodologies. These issues prompt questions about inclusivity, the development of contextualized frameworks, and the need for systematic investigations to deepen understanding and measurement of trust in AI. Also, it raises questions about the universal applicability of existing trust models and their relevance across different cultural contexts.

The evolution of trust relationships between users and AI systems also remains poorly understood. Trust appears to be a moving target, changing with technological advancement and societal expectations. \citet{benk2024twenty} raises some critical questions echoing these thoughts such as Is “trust” simply a convenient word? which often misses a definition, a foundational theory and often neglect the core concept of risk. Also, can we understand trust without outlining the context specific factors?

The trustworthiness of AI isn't solely determined by the technology itself \cite{lahusen2024trust}. It hinges on the intricate relationships between developers, public authorities implementing algorithmic decision-making (ADM) systems, and the citizens who are impacted. This interplay presents unique challenges. Developers create and maintain AI systems, yet their work is increasingly influenced by AI itself. Meanwhile, public authorities grapple with regulating AI on a global scale, even as they increasingly rely on it for decision support.

The broader impact of FAccT and AIES scholarship on AI trustworthiness is multifaceted. However, this community is still in its beginning in understanding broader impact of studying AI trustworthiness. While acknowledging their success in raising awareness, we could identify gaps in quantifying long-term impact, addressing global disparities, and exploring economic dimensions. Furthermore, we need more concrete, actionable policy recommendations stemming from this body of work and the crucial link between trustworthy AI and achieving the UN sustainable development goals.


\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/cooccurance_weights_tw_dims_network.png}
    \caption{PLEASE IGNORE}
    \label{fig:enter-label}
\end{figure}




\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.75\linewidth]{figures/TEMP_louvain.png}
    \caption{PLEASE IGNORE}
    \label{fig:louvain}
\end{figure}

The ISO definition of trustworthiness is based on the standard (5723:2022) which defines it as ``ability to meet stakeholders’ expectations in a verifiable way'' \cite{EU_AI_Ethics_Guidelines}. The characteristics of trustworthiness in the standard include, for instance, accountability, accuracy, authenticity, availability, controllability, integrity, privacy, quality, reliability, resilience, robustness, safety, security, transparency and usability. Some of these characteristics, are also a part of the National Institute of Standards and Technologies (NIST) AI Risk Management Framework \cite{NIST_AI_Risk_Management_Framework}. Both ISO and NIST provide definitions of these characteristics which is helpful in providing clarity on the use of these terminologies.

Moreover, there is a notable lack of focus on AI safety within the broader discourse on trustworthiness, despite its crucial role in ensuring the responsible development and deployment of AI technologies.

\footnote{The number in brackets denote the count of articles corresponding to specific dimension. Our frequency count includes articles belonging to multiple dimensions of ISO. For example, article A links trustworthiness to transparency and use explanations as a method communicate inner workings of a system. In this case, we increment the count both for explainability and transparency by one. }

==> sections/sec-values.tex <==
\section{Values linked to trustworthiness} - 
Values like Fairness, \textbf{Accountability} and
Transparency
Embedding Values in Artificial Intelligence (AI) Systems - we will use this paper for the narrative - note by Xu: I was unaware of this paper as it has not been mentioned before, so I have not worked through the framework of intended, embodied, or realized values

\begin{enumerate}
    \item Start off with explanation of what we mean with ``values'' here $\rightarrow$ public values theory, like Mark Moore, Jorgensen

    We stress the importance of the connection between AI trustworthiness research with practical policymaking. In the context, building upon the notion of values, the idea of \textit{public} values plays a crucial role. \citet{moore1997creating} views public values as outcomes that organizations strive to achieve, reflecting societal aspirations and the collective good, which guide and justify their existence and actions. In our case, we may view AI as the agent with which value van be provided to society, leading ultimately to perceptions of trust. Vice versa, through communicating trustworthiness, the implementation and working of the AI may provide or benefit public values. 

    
    \item Multiple trustworthy dimensions are values relevant in governance. 

    AI trustworthiness dimensions, as defined by the ISO, align with different categories of public values. Indeed, these values vary depending on the social relationship is referred to. For example, transparency for trustworthy AI would fall under public value of openness, which occurs in the relationship between provider--such as the public administration and its deployed algorithms--and its receiver, like stakeholders and the public \cite{jorgensen2007public}.   
    
    \item values are interrelated and can be grouped in ``bag of values'' 

    However, values are not mutually exclusive and have the tendency to interrelate. For instance, public values, like robustness, may commonly require the pursuit of adjacent values, such as reliability. This prompts multiple values to play an important role simultaneously, which in some way may lead to a ``bag-of-values'' to facilitate AI trustworthiness. 
    
    \item We analyzed quantitatively agaisnt these values 

    As the corpus analyses show, emphasis in the FAccT \& AIES literature is placed on understanding (e.g., transparency) and relying (e.g., quality) on the AI such that it becomes trustworthy. 
    \item in the results we see that...
    \item we also looked with GQM at these values
    \item in the results we see that...
    \item kind of contribution to this and that values are this and that (like through frameworks or technical tools, etc.)...
    \item conclusion
\end{enumerate}

\sid{I think your section is better suited in the section 4.5 and 7. The way you have structured the points it is interesting for the reader to know the outcome especially linked to challenges and recommendations you provide. Section 4.5 will be completed shortly. Please see how you can add your contribution streamlining the text there. It should be max 2 paras \~ 300 words. Till that time, feel free to add text here.}







